Cheetah: Accelerating Database Queries with Switch Pruning

Modern database systems are growing increasingly distributed and struggle to reduce query completion time with a large volume of data. In this paper, we leverage programmable switches in the network to partially offload query computation to the switch. While switches provide high performance, they have resource and programming constraints that make implementing diverse queries difficult. To fit in these constraints, we introduce the concept of data \emph{pruning} -- filtering out entries that are guaranteed not to affect output. The database system then runs the same query but on the pruned data, which significantly reduces processing time. We propose pruning algorithms for a variety of queries. We implement our system, Cheetah, on a Barefoot Tofino switch and Spark. Our evaluation on multiple workloads shows $40 - 200\%$ improvement in the query completion time compared to Spark.

==> sections/backup.tex <==
INtro
% Today, query optimization is mostly done in software
% %, either at the data source~\cite{XX} or 
% at the query server~\cite{Exadata, sparksql}. However, with the rapid growth of data volumes, it is increasingly challenging for software to keep up \mbox{with the performance requirements.}

% As some algorithms depend on hash-based partitioning of the data, FPGAs were also suggested for accelerating the partitioning task~\cite{}.
%\minlan{other offloading to fpga works}

Unlike traditional hardware accelerators which focus on FPGAs, GPUs, or SSDs, we implement \NAME on the emerging technology of programmable switches. Switches see the traffic from all partitions, they are used to move the data between storage and compute nodes anyways, and have exceptionally high bandwidth. Therefore, switches are prime candidates for accelerating the database operations.

%%%%%%%%%%%%SKYLINE%%%%%%%%%%%%%%
% For example, we can only decide whether a new \inputRow{} (e.g., (x1,x2)) is more valuable to store than an existing entry (y1,y2) after we compare x1,y1 and x2,y2. 
% However, switches cannot test on multiple conditions and write to memory (e.g., replace (y1,y2)) on the same stage. 
% Moreover, because of the limited number of comparison we can do (due to the limited number of stages), we also need to identify the best set of entries to store. 
 
%  For example, we can decide whether to store a new \inputRow{} (e.g., (x1,x2)) after we compare all the dimensions with an stored entry (e.g., when x1>y1 and x2>y2).  

To support the \skyline query, we store a cache of entries similar to \distinct queries. The challenge is that there is no strict ordering among all \inputRows{} (because we need to compare in multiple dimensions), so we need to compare an incoming packet to all the stored entries. This means we can only compare with a limited number of entries at each stage because we cannot do many comparison at each stage. 

Another challenge is that switches do not support read-test-write operation. We need to first compare an incoming \inputRow{} $x=(x_1,x_2)$ with a point on the switch $y=(y_1,y_2)$, and then make decision on whether we replace $y$ with $x$, prune $x$, or neither. However, such read-test-write operations cannot be implemented in one stage. Even if we implement the test and write in two stages, we still cannot go back to the previous stage to write $x$.\footnote{We can loop the packet back to the stage but it reduces the switch throughput.} 

Thus, the pruning efficiency of \skyline depends on how many points we can store and compare to, which in turn depends on the number of stages and the number of ALUs at each stage. 
%%%%%%%%%%%%SKYLINE%%%%%%%%%%%%%%


%The storage sends a stream of data to the aggregator via our switch. Each packet is identified with a sequence number that is observed by all parties. The switch and aggregator record the packet identifier of the last \textit{non-pruned} packet. Every fixed time interval (say, 1000 packets), the aggregator sends a message back to the storage, via the switch, with the last identifier that it observed. Seeing this packet, the switch checks if the reported identifier matches the identifier he recorded as the last non-pruned packet. If the identifier do not match, it drops the packet and otherwise forwards it to the storage. If the storage does not receive the acknowledging packet it retransmits all required packets. When seeing retransmitted packets (whose id is smaller than that stored on the switch), the switch forwards them without pruning or recording the data.

%\begin{table}%[H]
%           %\centering
%           
%           \captionsetup[subtable]{position = below}
%          \captionsetup[table]{position=top}
%           \hspace{-.3cm}
%           \resizebox{.85 \columnwidth}{!}{
%           \begin{subtable}[t]{0.3\linewidth}
%               \centering
%               \caption{\products}
%                \begin{tabular}{lcc}
%                \hline
%                \name&\seller&\price\\\hline
%                    Burger&McCheetah&4\\
%                    Pizza&Papizza&7\\
%                    Fries&McCheetah&2\\
%                    Jello&JellyFish&5\\
%                \hline
%                \end{tabular}
%               \label{tab:dimFFT}
%           \end{subtable}%
%           \hspace*{2.3cm}
%           \begin{subtable}[t]{0.3\linewidth}
%               \centering
%               \caption{\ratings}
%                    \begin{tabular}{lcc}
%                    \hline
%                    \name&\taste&\texture\\\hline
%                    Pizza&7&5\\
%                    Cheetos&8&6\\
%                    Jello&9&4\\
%                    Burger&5&7\\
%                    Fries&3&3\\
%                    \hline
%                    \end{tabular}
%                 \label{tab:dimGMM}
%           \end{subtable}
%           }
%           \caption{Running Example}\label{tbl:example}
%\end{table}

%To execute the query, \NAME first fetches a metadata stream that are directly related to the query. Based on these metadata, the switches prunes the set of data. 

%Consider having $\Gamma\in\set{\MIN,\MAX}$. We use our forward every row whose $z$ value exceeds $c$ and is reported as new by our \distinct algorithm.

% \minlan{clearly say what you support and what you do not}\ran{Is it not clear enough? I specifically wrote $>=$ and $f\in\set{\COUNT,\SUM}$. Any thoughts on how to make this clearer?}
% \minlan{CM means you update multiple entries?}\ran{Yes, we can keep each of Count Min's \matrixRows{} in a separate pipeline stage, or even up to 4 (\#ALUs) on the same stage. It's also possible to use a simple array (i.e., Count min with one row) but it will probably be less efficient in terms of pruning}
%Only if the Count Min reports that $\Gamma(z)$ exceeds the threshold $c$ we forward the row identifier $y$ to the aggregator. The aggregator requests all rows with value $y$ and \mbox{checks the condition again.}
%

%To reduce the number of times we report the same value $y$ to the aggregator, we add every reported entry to our \distinct algorithm explained in Section~\ref{sec:distinct}. 


% Frequency sketches with one-sided errors such as the Count Min sketch~\cite{} allow us to safely prune the data.

%It is often useful to apply a filter based on the result of a stateful computation. For example, SELECT buyedID FROM Customers GROUP BY buyedID HAVING MAX(price) $>=$ 1000 can be used to compute all customers that have purchased a product that cost at least $\$1000$. \NAME first filters the rows for which the price is lower than the threshold and then adds 


%This allows us to request only the rows that belong to the aggregates which are reported to meet the filtering criteria. Note that this gives a false-negative free approach and thus we deterministically guarantee the correctness of the operation.
%Only if the Count Min reports that the frequency exceeds the threshold $c$ we forward the row to software and otherwise prune it. For additional pruning, we can insert the current row into our \distinct solution and prune future instances of it. 



%For filtering based on \groupby of MAX or MIN we propose the following solution; we explain it for MAX operations while MIN is symmetric. 
%Consider the query SELECT buyedID FROM CUSTOMERS GROUP BY buyedID HAVING MAX(purchaseValue) $>=$ 10 that finds all buyers that purchased an item worth at least $$


% \minlan{Why this false positives is worse than fingerprint collision?} \ran{False positives mean that the output is incorrect. Fingerprint collisions within the same row \emph{create false positives} and therefore our analysis considers what we can support while guaranteeing that there are no same-row fingerprint collisions}
%A false negative in our case means a row that has appeared, but the switch thinks that it has not. In this case, the switch may not prune the duplicate row. Instead, the query server can run the distinct selection on the pruned set and remove the few redundant entries.

%\begin{proof}
%We use the bound on the maximum number of distinct elements that are mapped into a row presented in %Theorem~\ref{thm:distinct}. Specifically, we had that since $D > d\ln(200d)$ then with probability %$99$\% we have that no row processes more than $e\cdot D/d$. That is, if we denote by $I$ this event, %we have $\Pr[I]\ge0.99$. \emph{Conditioned on $I$}, we have that each redundant row is pruned with a %probability of at least $\min\set{w/\max\set{D_i},1}\ge \min\set{\frac{w \cdot d}{D\cdot e},1}$. %Therefore, we conclude that in expectation we prune at least $\Pr[I]\cdot \min\set{\frac{w \cdot %d}{D\cdot e},1} = 0.99\cdot \min\set{\frac{w \cdot d}{D\cdot e},1}$.
%\end{proof}
%
%Design overview
%\minlan{
%limited associativity LRU-like structure that adapts to the current traffic and tries to store %elements that are more likely to appear again. If an element that is represented in our structure %appears once more we will be able to identify that and prune it.
%}
%
%Design benefits
%We can work with a small number of stages, and we can have 
%
%matrix, 
%
%LRU
%
%false positive proof on finger print
%
%
%For a false-positive free\minlan{not really}\ran{Not sure what you mean by that. As long as that %there are no fingerprint collisions between items that are mapped to the same row we have no false %negatives. The analysis we have is on how large should the fingerprints be such that with a high %probability this does not happen. This is exactly the same probabilistic guarantee that we give for %TOP N.} set representation, we store a cache of fingerprints of seen items. If an item's fingerprint %is in the cache we prune it and otherwise pass it to the software. 
%Specifically, we create a $d\times w$ matrix of observed entries. Initially, all cells are empty. %Whenever an item $x$ arrives, we use a hash function to map it into one of the $d$ matrix rows. The %packet then traverses the row; at each location we check whether the cell has the identifier of $x$. %If so, we mark the packet for drop. Otherwise, if the cell is empty, we insert $x$ into the cell.
%If a packet traversed the entire row without being marked for a drop we forward its value to the %software aggregator. 
%
%Intuitively, the matrix approach has two advantages: First, it reduces the number of per-item %comparison to $w$ which makes it suitable for programmable switches. Second, it reduces the chance of %false positives and thereby allow shorter fingerprints. This is because fingerprint collisions for %items that are hashed to different rows do not result in false positive and thus we tune the %fingerprint size to avoid collisions \emph{only within the same row}.
%For example, for any stream of size $m=100M$, if $w=16$ and $\delta=0.01\%$, we need need %fingerprints of (at least) $44$ bits.\minlan{Change to the dinstinct element numbers}\ran{not sure %what you mean by that} We prove the pruning ratio in the Appendix.\ran{this is not clear to me. The %pruning ratio analysis is only for random-order stream, which is something we should mention. IMO we %also need to state the results here.}
%
%% We prove the pruning ratio follows the theorem: 
%% \begin{theorem}
%% %Let $\mathcal M$ be defined as in Theorem~\ref{thm:distinct}, and consider
%% Consider a random order stream with $D > d\ln(200d)$ distinct entries\footnote{It's possible to %optimize other cases as well, but this seems to be the common case.}. Our algorithm, configured with %$d$ rows and $w$ columns is expected to prune at least $ 0.99\cdot \min\set{\frac{w \cdot d}{D\cdot %e},1}$ fraction of the duplicated entries.
%% \end{theorem}
%
%To further increase the pruning ratio, we can implement an LRU-based eviction \red{Jiaqi said he %believes that this is doable, we need to make sure}.
%That is, if $x$ is stored in some cell in the matrix row it is hashed to, we will drop the packet; if %$x$ is not stored and there exists an empty cell in the row, we add $x$ to it; at any case we keep %the row sorted by the most recent arrival time. That is, if the row is full and $x$ does not have a %counter the evicted element will be the done that we have not seen for the longest time. 
%\ran{I don't think that it is good to remove the analysis altogether. It makes the reader think that %this is a heuristic algorihms with no correctness guarantees. I suggest that (1) we leave the formula %on how to set the parameter and (2) leave a statement of the correctness theorem. The proof can be %deferred to an appendix.}
%
%\ran{
%My understanding is that on random order streams LRU can only improve the pruning rate (although it %may be identical at the worst case).
%In adversarial streams (if the adversary knows we are using LRU) the result can be arbitrarily bad in %terms of pruning, but the algorithm still provide correctness.}

% Therefore, we introduce a \emph{probabilistic} pruning algorithm which provides all distinct \inputRows{} except with a small, user-defined, probability $\delta$.(We set $\delta$ as XX in our prototype.)

% \distinct query means that the switch must provide a superset of all the distinct values in the input. To that end, we can only prune points that have surely appeared before. Therefore, commonly used set representations such as Bloom filters are inadequate as they have false positives which may lead to pruning of rows that have not appeared before and to the failure of serving the query. Hence, we need to design a set representation with no false positives. 
    % As a benchmark we propose to store the first values and the trace and prune them if they appear again. 
    % In contrast, our algorithm uses hashing, fingerprinting and   
    
    
    %find the {\em best} candidates from a set where there are multiple metrics (dimensions) of goodness. 
%For example, consider selecting an hotel given the ratings in Booking.com and Tripadvisor.com. If hotel $x$ received lower scores than $y$ on both rankings, we may choose to examine $y$ and not $x$.

% Consider an input point $(x_1,x_2)$ and a point stored on the switch $(y_1,y_2)$; we can prune $x$ if it is dominated by $y$, but if $y$ is dominated by $x$ we may want to store $x$ on the switch instead of $y$ to get better pruning. However, replacing $y_1$ and $y_2$ together if and only if $(y_1<x_1)$ \emph{and}  $(y_2<x_2)$ requires the read-after-write operation which is not possible to do in one stage. 

==> sections/oldAlgs_includingGROUPBY.tex <==

\newpage\ \newpage

\parab{Primitive \#1: Cache Partial Data on the Switch.}\\
The switch has limited memory and per-packet processing ability. In our algorithms we store a small number of entries that reflect past elements, and use them to consider whether to prune new ones. 
For example, our \distinct solution stores a cache of recent (distinct) elements, as these are more likely to appear again than previous ones (an LRU approach).

The choice of \emph{which} items to store depends on the query, but as a general rule we prefer recent data over old one (as in caching algorithms) and \emph{prominent} elements that are more likely to assist in pruning over those that do not. These principles occasionally conflict, and our algorithms must balance between the approaches.
For example, if we compute the most profitable transaction per seller (a \groupby query), we reflect both the value of an entry and its recency to determine which transactions to store.


\parab{Primitive \#2: In-switch Data Partitioning.}\\
Since we do not need to get the exact query results, we can use the limited stages and ALUs to best filter out data. For example, we can divide the data into partitions, so that each incoming entry only compare with the stored values in this partition. 
%We can also use a \emph{projection} where we map a high-dimensional data point into a single scalar value to allow efficient comparison. 

\parab{Primitive \#3: Data Projection.}\\
The output of some queries depends on the value of multiple columns (e.g., in \skyline), or variable-width columns (e.g., \join where the keys are strings). The simplest type of projection is hashing -- instead of looking at the actual keys we can use fixed-width hashes of them. Another projection is mapping high-dimensional points into scalars using a monotone function. For example, in a \skyline query with two dimensions, a point $x$ dominates $y$ if $(x_i>y_i)\wedge(x_2>y_2)$. 
Ideally, if $y$ is cached, we would want to replace it with $x$ to improve the future pruning. However, such multi-read;multi-write operation is hard to implement on programmable switches. Instead, we can store $h(y)=y_1+y_2$ before the point itself. If $x$ dominates $y$ we surely have $h(x)>h(y)$ and therefore can write $\max\set{h(x),h(y)}$ on the first step and if $h(x)>h(y)$, replace $y$ on the next step.

\parab{Primitive \#4: Approximate Unsupported Functions.}\\
There is only a limited set of operations we can do at switches. 
For example, the switch is often incapable of some arithmetic operations except on power-of-two numbers {(e.g., division, multiplication, log).}
We leverage the switch TCAM, SRAM, and ALUs to approximate these functions when needed.

\parab{Primitive \#5: Partial Query Pruning.}\\
Due to the switch limitations, we may not be able to prune all parts of a query. 
For example, consider the following query. 
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT * FROM Products              WHERE texture > 4 AND name LIKE e\%s 
\end{lstlisting}
If the switch cannot evaluate (\name LIKE e\%s), we can prune all entries for which texture $\le 4$ and leave checking \name to the master node.

\begin{comment}
\parab{Limited pipeline stages and ALUs:} 
Since we do not need to get the exact query results, we can use the limited stages and ALUs to best filter out data. For example, we can divide the data into partitions, so that each incoming entry only compare with the stored values in this partition. We can also use projection where we map a high-dimensional data point into a single scalar value to allow efficient comparison. 

\parab{Memory and bit constraints:} 
As our goal is to prune entries, we capture an approximate view of the past data to assess whether the current entry should be pruned. Our  view allows us to get bounds on the actual data and use them for pruning. For example, if a query asks for all keys that appear more than $100$, \NAME{} will forward all keys for which its computed lower bound is no less than $100$. This way we are guaranteed to never miss an output key while the master removes all non-pruned keys for which the frequency is \mbox{lower than $100$ (false positives).}

\NAME provides the approximate view by caching and compression. For example, we propose a value-aware key-value cache for our \groupby operation. The cache tends to store newer keys, but also ones with values that are more likely to allow better pruning.
To reduce the number of bits, we leverage fingerprinting and encoding only a subset of the columns (leaving the other \mbox{columns for the master to process).}

\parab{Function constraints:}
We do not need to implement all the database functions at switches but only offload those that fit in the switch programming model while leaving the remaining to the master. 
\end{comment}


% We note that if the resulting formula is a tautology (e.g., in the case of WHERE $\texture > 4 $ OR \name LIKE e\%s ), \NAME will not be able to perform any pruning.

%Nevertheless, if the condition can be expressed expressed as $\phi \wedge \psi$ for Boolean expressions $\phi ,\psi$, where $\phi$ is computable on the datapath,
%\NAME will compile filtering based on $\phi$ alone. This allows pruning of rows that surely do not satisfy $\phi \wedge \psi$ and thus reducing the data scale. 

\subsection{Distinct Selection}\label{sec:distinct}
The \distinct query selects all the distinct values in a \inputCols{} subset. 
\mbox{For example,the query}
%SELECT DISTINCT \seller FROM \products 
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT DISTINCT seller FROM Products 
\end{lstlisting}
may return (Papizza, McCheetah, JellyFish). 
To prune for \distinct queries, the basic idea is to store all the past values in the switch. When the switch sees a new \inputRow{}, it simply checks if the new value matches any past values. If so, the switch drops this \inputRow{}; if not, the switch forwards it to the master node. However, storing \inputRows{} on the switch may take too much memory.

To reduce memory usage, an intuitive idea is to use Bloom filters~\cite{bloom1970space} (BFs). However, BFs have false positives. This means that the switch may drop \inputRows{} even though their values have not appeared.

Therefore, we need a data structure that ensures no false positives but can have some false negatives. The query server can then rerun the distinct query to remove the false negatives. Caches match this goal. 

We propose to use a $d\times w$ \emph{matrix} in which we store \emph{fingerprints}. Each entry, regardless of its number of columns, is mapped to a fixed-length fingerprint to save space and comparisons. Every \matrixRow{} serves as an LRU cache that stores the last $w$ fingerprints mapped to it.
When an \inputRow{} arrives, we first \emph{hash} to $\set{1,\ldots,d}$, so that the same \inputRow{} always maps to the same \matrixRow{}. \NAME then checks if the current \inputRow{}'s fingerprint appears in the \matrixRow{} and if so prunes the packet. We also do a rolling replacement of the $w$ entries by replacing the first one with the new entry, the second with the first, etc., to implement LRU. 
% \footnote{
% We can further reduce the required number of stages by using FIFO instead of LRU on those switches which supports \emph{same-stage} ALUs to share the SRAM space.}

% Intuitively, as long as there are no fingerprint collisions \emph{within the same \matrixRow{}} the algorithm cannot mistaken the current entry as duplicate if it has not appeared before. 

%To further increase the pruning rate we adopt an LRU-like structure in which each \matrixRow{} implements an LRU cache. That is, for each \matrixRow{} the algorithm stores the fingerprints of the last $\le w$ distinct elements hashed to it.
By using multiple \matrixRows{} we achieve two benefits: (1) We reduce the number of per-packet comparisons to allow implementation on programmable switches (2) We decrease the number of bits required for the fingerprints as each item is only required to have a distinct fingerprint \emph{within the \matrixRow{}}.

% \begin{figure}[t]
%     \centering
%     %\begin{subfigure}[Simple mode]{}
%     {\includegraphics[width=0.99\linewidth]{Figures/Distinct_IllustrationV5.png}}
%     \caption{An illustration of the algorithm on the following sequence of website accesses: %(cnn.com,cnn.com,nbc.com,nba.com,cnn.com,nhl.com). 
%     (cnn,cnn,nbc,nba,cnn,nhl). 
%     The fingerprints are $f(\mathit{cnn}) = 17, f(\mathit{nbc}) = 91,  f(\mathit{nba}) = f(\mathit{nfl}) = 33,  f(\mathit{nhl}) = 64$ and all except "nba" are hashed into the second \matrixRow{}. On the second and third appearances of cnn, \NAME sees $17$ in the second \matrixRow{} and is able to prune the packet. If the next \inputRow{} would ask for "nbc", we will not find it in the matrix and it will be removed by the aggregator and not pruned on the switch.
%         ~\label{fig:distinct}}
%       % \vspace*{-5mm}
% \end{figure}

We provide a rigorous analysis of this scheme in Appendix~\ref{app:distinct}. The analysis leverages a balls and bins theory to derive bounds on the \emph{sum of square loads}, where each load is the number of distinct elements mapped into a \matrixRow{}. It then considers the number of distinct elements we can support without having same-row fingerprint collisions. For example, if $d=1000$ and the error probability $\delta=0.01\%$, we can support up to $500M$ distinct elements using $64$-bits fingerprints \emph{regardless of the data size}. Further, this does not depend on the value of $w$. Additionally, we analyze the expected pruning rate in random-order streams and show that we can prune at least an $\Omega\parentheses{\frac{w \cdot d}{D}}$ fraction of the entries, where $D$ is the number of distinct elements. 
% \minlan{need to comment on fingerprints collision in one sentence}\ran{not sure what you mean by that? As explained, 64-bit fingerprints ensure no same-row collisions with prob. 99.99\%}

% \minlan{With perfect switch, with the same amount of memory, LRU has better pruning, (but more stages); FIFO needs fewer stages, 
% With Tofino you should do LRU....}


\subsection{Skyline}
The Skyline query~\cite{borzsony2001skyline} returns all points on the Pareto-curve of the $D$-dimensional input. 
Formally, a point $x$ is dominated by $y$ only if it is dominated on all dimensions, i.e., $\forall i\in\set{1,\ldots, D}: x_i\le y_i$. 
%Further, $x$ is strongly dominated by $y$ if $\forall i, x_i < y_i$. 
The goal of a \skyline query is to find all the points that are not dominated in a dataset.\footnote{For simplicity, we consider the case of maximizing all dimensions. We can easily extend the solution to support minimizing all dimensions with small modifications.} 
For example, the~query 
%SELECT \name FROM \ratings SKYLINE OF \taste, \texture 
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT name FROM Ratings          (*\bfseries SKYLINE*) (*\bfseries OF*) taste, texture 
\end{lstlisting}
could return (Cheetos, Jello, Burger). 

% You could do x1 <- max(x1,y1) and x2 <- max(x2,y2),
% what you can do is have this conditional branching that replaces x1 only if the condition on x2 holds simultaneously. 
% What you can't do*.
% There are two possible encodings:
% 1. you have x1 and x2 on the same stage, then this requires same-stage conditional branching, which is prohibited.
% 2. you have x1 on one stage and x2 on the next, then by the time you compare x2 to y2 you'd need to recirculate to replace x1.

Because skyline relates to multiple dimensions, when we decide whether to store an incoming entry at the switch, we have to compare with all the stored entries because there is no strict ordering among them. For each entry, we have to compare all the dimensions to decide whether to replace it. But the switch does not support conditional write under multiple conditions in one stage. The two constraints together make it challenging to fit \skyline queries on the switch with a limited number of stages. 

To address this challenge, we propose to map each high-dimensional \inputRow{} into a single numeric value.
We define a function $h:\mathbb R^D\to\mathbb R$ that gives a single \emph{score} to $D$-dimensional points. We require that $h$ is monotonically increasing in all dimensions to ensure that if $x$ is dominated by $y$ then $h(x)\le h(y)$. In contrast, $h(x)\le h(y)$ does not imply that $x$ is dominated by $y$.

The switch stores a total of $w$ points in the switch. Each point $y_{(i)}, i=1..w$ takes two stages: one for $h(y_{(i)})$ and another for all the dimensions in $y_{(i)}$. When a new point $x$ arrives, for each $y_{(i)}$, the switch first checks if $h(x)>h(y_{(i)})$. If so, we replace $h(y_{(i)})$ and $y_{(i)}$ by $h(x)$ and $x$. Otherwise, we check whether $x$ is dominated by $y_{(i)}$ and if so mark $x$ for pruning \mbox{without changing the state.}
Note that here our replace decision is only based on a single comparison (and thus implementable at switches); our pruning decision is based on comparing all the dimensions but the switch only drops the packet at the end of the pipeline (not same stage action). 

If $x$ replaced some $y_{(i)}$, we put $y_{(i)}$ in the packet and continue the pipeline with the new values. We use a rolling minimum (according to the $h$ values) and get that the $w$ points stored in the switch are those with the highest $h$ value so far are among the true skyline.% 

Now the question is which function to use for $h$. We can use {\em sum}, which is defined as $h_S(x)=\sum_{j=1}^D x_j$, but it is biased towards the dimension with a larger range (Consider one dimension  ranges between $0$ and $255$ and another between $0$ and $65535$).  
%For example, consider a query on two \inputCols{} where the first ranges between $0$ and $255$ and the second between $0$ and $65535$. In this case, the sum heuristic will favor $x=(1,65500)$ over $y=(256,65200)$. However, the volume of the region dominated by $x$ and not $y$ is tiny compared to the volume covered by $y$ and not $x$.
Another option is to use {\em product}, which is defined as $h_P(x)=\prod_{i=1}^D x_i$. Product addresses the issue of dimensions with different magnitude but is hard to implement on switches because it requires large values and multiplication. %The main issues are that the result could be excessively large for the switch to handle (e.g., the product of five $64$-bit fields may require over $300$ bits) and that the switch may not support multiplication.
Instead, we use Approximate Product Heuristic (APH) which uses the monotonicity of the logarithm function to represent products as sum-of-logarithms and uses the switch TCAM and lookup tables to approximate the logarithm values (see more details in Appendix~\ref{app:skyline}).
%In Appendix~\ref{app:skyline} we discuss how to implement the 

%\minlan{Moreover, the product heuristic is \emph{optimal} in terms of the pruning rate for random points on the domain (when $w=1$). }
%\ran{I guess you want to remove this sentence? I don't mind. It's just trying to give intuition as to why product will be better (the product reflects the $d$-dimensional volume dominated by the point.}

% We illustrate the difference between the two heuristics in Figure~\ref{fig:skyline}.
% \begin{figure}[t]
%     \centering
%     %\begin{subfigure}[Simple mode]{}
%     {\includegraphics[width=0.99\linewidth]{Figures/skylineIllustration.pdf}}
%     \caption{When the dimensions of the \skyline queries have different magnitudes, the SUM heuristic may be biased towards the dominant direction dimension. This illustrates the contours of the SUM and PRODUCT heuristic over two dimensions, ranging $[0,255]$ and $[0,4095]$. As can be seen, the SUM heuristic prefers point A over B, although the volume covered by it is much smaller.
%         ~\label{fig:skyline}}
%       % \vspace*{-5mm}
% \end{figure}

%So how do we make product work in the switches. We cannot complex computation, and have limited number of bits. 
%The number is too large, and we use match 
%\minlan{correct terms, col, row, entry, dimension, points}



%\ran{hmm, does that actually work? should we use $f$ just on the most significant 16-bits? maybe use 
%$\begin{cases} f(x \& FFFF0000)+16 &\mbox{if $x\ge2^{16}$}\\
%f(x \& 0000FFFF) &\mbox{otherwise}
%\end{cases}
%$
%?}
%For example, if $x$ is a $32$-bits integer first find the location of its most significant $1$-bit $\ell=\ceil{\log_2 x}$ and use $\widehat{H_P(x)}\triangleq f(x[\min{0,\ell-16},\ell])$. That is, we apply $f$ on the 16-bits 
%Simple algebra shows that this mapping can produce estimates $\widehat{H_P(x)}$ that satisfy $H_P(x) - H_P(x)(\alpha-1)/\beta\le \widehat{H_P(x)}\le H_P(x) + H_P(x)(\alpha-1)/\beta$.

\subsection{Top N}
In a \topn query (with an ORDER BY clause), we are required to output the $N$ \inputRows{} with the largest value in the queried \inputCol{}.\footnote{In different systems this operation have different names; e.g., MySQL supports LIMIT while Oracle has ROWNUM.} For example, the query
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT (*\bfseries TOP*) 3 name, texture FROM Ratings ORDER BY taste 
\end{lstlisting}
%SELECT TOP 3 \name, \texture FROM \ratings ORDER BY \taste 
may return (Jello 4, Cheetos 6, Pizza 5). Pruning in a TOP N query means that we may return a superset of the largest N \inputRows{}. 
The intuitive solution is to store the $N$ largest values, one at each stage. We can then compare them and maintain a rolling minimum of the stages. 
%the $N$-largest points seen so far and prune any point smaller than the $N$'th largest observed value. If $N$ is small then a simple rolling minimum of $N$ stages will allow you to do exact filtering. 
However, when $N$ is much larger than the number of stages (say 100 or 100), this approach does not work. We propose both deterministic-guarantee and probabilistic-guarantee algorithms as described below.

\parab{Deterministic algorithm:}
The deterministic approach first computes the minimal value $t_0$ among the first $N$ entries. Afterward, we can safely filter out everything smaller than $t_0$. It then tries to increase the threshold by checking how many values larger than $t_1$ we observe, for some $t_1>t_0$. Once $N$ such entries were processed, we can start filtering elements smaller than $t_1$ and so on. Specifically, for hardware friendliness, we use $t_i=2^i\cdot t_0$.
%\minlan{How does the switch runs this?}\ran{we can count the number of elements larger than $2t_0$, $2^2t_0,\ldots 2^c t_0$ using $\approx c$ stages. Then if we have $N$ elements larger than $2^i t_0$ we can start filtering based on that}%this is a meta-algorithm that doesn't explain how to set $t_1$ after fixing $t_0$. There are many possible implementations. For example, you can take the minimum of the first $N$ entries larger than $t_i$ as $t_{i+1}$. Alterna}
        
%The first starts as the benchmark algorithm by setting a threshold of the minimum of the first $N$ points, but increases the threshold over time while ensuring correctness. 
%
%
%    
%    
%In a TOP N query, the algorithm returns the N rows with the largest value on the queried column. For %example, one may wish to find the $100$ cheapest hotels in Honolulu or the $100$ hotels that are %closest to the beach.

\parab{Probabilistic algorithm:}
To further improve the pruning ratio, we also introduce a  probabilistic algorithm which leverages the balls and bins framework to randomly partition the input into bins while ensuring that if the maximum load is not large we successfully pass all top $N$ points. The algorithm may err with a small probability $\delta$ configurable by the user (e.g., $\delta=0.01\%$) but provides superior pruning rate compared to the deterministic solution.

The randomized approach aims to return a superset of the expected output with high probability. For example, we may configure it to guarantee that with probability 99.99\% \emph{none} of the $N$ \outputRows{} is pruned.
To that end, we use a $w\times d$ matrix which is initialized to all $-\infty$. Whenever a new value arrives, we use a hash function to map it into one of the $d$ \matrixRows{}. In each \matrixRow{} we store the $w$ largest entries that were mapped to it using a rolling minimum. If the current point is smaller than all $w$ values we compare it to then we prune it. The algorithm is illustrated in Figure~\ref{fig:topn-example}.

        \begin{figure}[t]
    \centering
    %\begin{subfigure}[Simple mode]{}
    {\includegraphics[width=0.99\linewidth]{Figures/TopN_IllustrationV2.png}}
    \caption{\topn example on a stream (7,4,7,5,3,2). The \inputRow{} $3$ was mapped to the third \matrixRow{} and pruned as all stored values were larger. In contrast, $2$ was mapped to the second \matrixRow{} and is not pruned. The matrix dimensions are chosen so that with high probability none of the \topn \mbox{\inputRow{} will be pruned.}
        ~\label{fig:topn-example}}
        \vspace*{-2mm}
\end{figure}

The proper $(w,d)$ configuration of the algorithm (given $N$, the desired error probability $\delta$, and the hardware resource constraints) is quite delicate.
In Appendix~\ref{app:topn}, 
analyze how to set $w$ given a constraint on $d$ (which dominates the per-stage SRAM usage) or vice versa that simultaneously optimizes the expected pruning rate. We also show that we achieve the best pruning rate when the matrix size $d \dot w$ is minimized (if there is no constraint on $d$ or $w$). 

%both the SRAM utilization and 
%\minlan{What's your optimization function exactly? You have two goals here}\ran{This is the cool part. It turns out that both the space and the pruning rate are monotone in $(d\cdot w)$. (space being monotonically increasing, pruning rate monotonically decreasing). This means that if we have no constraint on $d$ and $w$, we can minimize the space and maximize pruning at the same time. Basically, I'm solving "minimize $(d\cdot w)$ such that the algorithm finds top N with prob 1-delta". This optimizes both metrics at the same time, and is only infeasible if we cannot afford these $w$ values (in terms of number of stages) or $d$ values (in terms of space)}
% We also provide an analytic solution to this optimization problem. For example, if we constrain $w$ to $5$ (hardware stages) we need to set $d$ to $1472$ ($\approx$10KB memory per stage), we will need  for finding the top 250 with probability 99.99\% and get expected pruning of 99.3\% out of a 10M sized input. If we are unconstrained, we should use $w=17$ and $d=134$ which gives 99.8\% pruning.


\subsection{Groupby}
The \groupby operation requires summarizing all \inputRows{} that share the same value on a subset of the \inputCols{} that are grouped. For example, the query
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT seller, MAX(price) FROM Products GROUP BY seller
\end{lstlisting}
%SELECT TOP 3 \name, \texture FROM \ratings ORDER BY \taste 
may return (McCheetah 4, Papizza 7, JellyFish 5).
                %\begin{tabular}{lcc}
                %\hline
                %\name&\seller&\price\\\hline
                %    Burger&McCheetah&4\\
                %    Pizza&Papizza&7\\
                %    Fries&McCheetah&2\\
                %    Jello&JellyFish&5\\
                %\hline
                %\end{tabular}
%This means that for reducing the data scale it is possible to \emph{merge} rows. For example, if the query is SELECT user, SUM(value) AS totalPurchases GROUP BY user, and the data is $\angles{x,5},\angles{y,3},\angles{x,4},\angles{z,6},\angles{x,2}$, it can be reduced to $\angles{x,9},\angles{y,3},\angles{z,6},\angles{x,2}$ without changing the output of the query.\minlan{change to the same example} 

An intuitive solution is to maintain an entry of the seller and price information for incoming packets at the switch and compute the maximum to reduce the data scale. However, we may not have enough memory to store an entry for each key (seller).

Instead, we design a sketch that allows us to prune entries which are smaller than the previously processed maximum. The sketch is a $d\times w$ matrix where each cell contains a key (e.g., seller) and a value (e.g., price).
The sketch utilizes $w$ hash functions $h_1,\ldots,h_w$ that map keys into $\set{1,\ldots,d}$.
For each new entry $(k,v)$, we compute its $w$ hash values $\{h_i(k)\}$. If one of the $w$ hashed locations stores the same key $k$ and its value is larger than $v$, we prune the packet. We also update all the $w$ entries with the new entry $(k,v)$.  
As an optimization, if there exists $i$ for which the $i,h_i(k)$ entry has $(k,v')$ for some $v'>v$ then we will set $h_{i+1}(k),\ldots,h_w(k)$ to $(k,v')$ rather than $(k,v)$.
Figure~\ref{fig:sketch} shows an example of how we run the \groupby algorithm.
\begin{figure}[t]
    {\includegraphics[width=0.99\linewidth]{Figures/sketch3.png}}
    \caption{Groupby example: $d=w=3$ and the data contains $(x,5),(x,2),(y,2),(y,1),(x,3)$. All but the first appearances of $x$ and $y$ are successfully pruned. Here, $h_1(x)=h_1(y)=2; h_2(x)=1;h_3(y)=2;h_3(x)=1$.
        ~\label{fig:sketch}}
 %       \vspace*{-5mm}
\end{figure}
%Instead, we reduce the amount of rows by storing an on-switch cache of counters and evicting them whenever we run out of space.
%For example, the data $\angles{x,5},\angles{y,3},\angles{x,4},\angles{z,6},\angles{x,2}$ can be reduced to $\angles{x,9},\angles{y,3},\angles{z,6},\angles{x,2}$ without changing the output of the query.
%\ran{Which cache design can we implement on the switch? A simple array would work but there has to be something better.}

%Ran: I'm so sorry, the paragraph below seems obsolete and detached from our current algorithm
%However, this requires storing the current values of each user\minlan{user? you mean key?} on the switch. To that end, we use a cache that allows us to store several entries for efficient merging.\minlan{how does cache work on w*d matrix?Do you use LRU here?} Whenever we run out of space, or if the counters are about to overflow \minlan{how do you tell? what counter do you mean? you just store (k,v)}, we evict the entries to the software.
%
% Another extremely common database operation is GROUP BY, where we look at a subset of the columns and aggregate over the others. For example, if we have a table of transactions with two columns -- buyer identifier and purchase value, we may run SELECT buyer, SUM(value) AS totalPurchases GROUP BY buyer to compute the overall amount of money spent by each buyer. 
%he same design also applies to additional aggregation functions %uch as MIN, MAX, and PRODUCT. For PRODUCT, 
%e evict counters earlier\minlan{how early, what do you mean} to %avoid overflows. 
%To support AVERAGE, we also compute the number of repetitions of %the grouped-by \inputCols{} and the sum.

%\subsection{HAVING clause}



\subsection{Join}\label{subsec:join}
In a \join operation we combine two tables based on the target \inputCols{}.\footnote{We refer here to INNER JOIN, which is SQL's default. With slight modifications, \NAME can also prune LEFT/RIGHT OUTER joins.} For example, the query
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT * FROM Products JOIN Ratings    ON Products.name = Ratings.name
\end{lstlisting}
gives
                \begin{tabular}{lcccc}
                \hline
                \name&\seller&\price&\taste&\texture\\\hline
                    Burger&McCheetah&4&5&7\\
                    Pizza&Papizza&7&7&5\\
                    Fries&McCheetah&2&3&3\\
                    Jello&JellyFish&5&9&4\\
                \hline
                \end{tabular}.\\
%As a baseline we propose to stream table $A$ while computing a Bloom filter for it, and then stream $B$ while pruning entries for which the filter returns false.
%In contrast, our 
In the example, we can save computation if the switch identifies that the key "Cheetos" did not appear in the \products table and prune it. 
%Alas, tracking the exact set of observed keys is infeasible and therefore \NAME approximates it using Bloom filters.

We use Bloom Filters to track observed keys. 
Specifically, consider joining tables A and B on \inputCol{} (or \inputCols{}) C. Initially, we allocate two empty Bloom filters~\cite{bloom1970space} $F_A, F_B$ to  approximately record the observed values
(e.g., \name) by using an \inputCol{} optimization to stream the values of C from both tables. Whenever a key $x$ from table A (or B) is processed on the switch, \NAME adds $x$ to $F_A$ (or $F_B$).
%(2) prunes the packet if $x\notin F_B$ ($F_A$). 
%Intuitively, if a key appears in both tables we will forward \emph{its second appearance} to the aggregator and prune the first one (unless we get a false positive from the Bloom filter). 
%Whenever the aggregator receives a (non-pruned) key, it issues a request for all \inputRows{} from that key from both tables. 
Then, we start a second pass in which the switch prunes each packet $x$ from A (respectively, B) if $F_B$ ($F_A$) did not report a match.
As Bloom Filters have no false negatives, we are guaranteed that \NAME does not prune any matched entry. The false positives in Bloom Filters only affect the pruning ratio. 
% Our algorithm is illustrated in Figure~\ref{fig:join}.
%         \begin{figure}[t]
%     \centering
%     %\begin{subfigure}[Simple mode]{}
%     {\includegraphics[width=0.99\linewidth]{Figures/Join_IllustrationV3.png}}
%     \caption{An illustration of the algorithm on two tables: $A$, which contains $x$ and $y$ and $B$ which contains $y$ and $z$. \NAME{} creates  the Bloom filters for $A$ and $B$ and on the second pass the switch forwards both $y$ entries as they match the filter and prune $x$ which does not. $z$ is not pruned due to a false positive in $F_A$ is removed by the master node.
%     %\NAME adds $x$ to $F_A$ when it arrives and prune it as $F_B$ reports that it was not observed for $B$. Then $y$ arrives from table $A$ and gets pruned as well. When $B.y$ arrives, $F_A$ reports a match and $y$ is forwarded to the aggregator which asks for all its \inputRows{} in both $A$ and $B$. Finally, $B.z$ arrives; although it does not match an entry in $A$, a false positive in the Bloom filter $F_A$ causes the packet to be forwarded. The aggregator will then request $z$'s \inputRows{}, find out that no such entry exists for $B$, and discard it \mbox{from the output.}
%         ~\label{fig:join}}
%       % \vspace*{-5mm}
% \end{figure}
%Specifically, our solution allocates a Bloom filter for each of the joined tables. Whenever an entry from one table arrives, the switch adds its key to the table's Bloom filter. It then checks whether the Bloom filter \emph{of the other table} reports the key as observed. As Bloom filters have no false positives, we are allowed to prune the packet 

%Our algorithm streams the fingerprints of all rows in $A$ and $B$ to the switch and creates Bloom filters for both. Then the entries of $A$ and $B$ themselves are streamed while pruning any row that does not pass the filter.
%\subsubsection{Join pruning}
%Specifically, assume that two tables $A$ and $B$ are joined on a shared column $c$. Our solution starts by streaming $c$ from both columns to the switch. The switch then computed a Bloom filter $A_c$ of the $c$ values that appeared in $A$ and similarly $B_C$. Next, both $A$ and $B$ are streamed in arbitrary order. Whenever a row $r_A$ from $A$ is processed, it is pruned unless its $c$-value is reported as existing by $B_c$ and vice versa.
%\begin{figure*}[t]
%    {\includegraphics[width=0.99\linewidth]{Figures/join.png}}
%    \caption{
%        ~\label{fig:join}}
%       % \vspace*{-5mm}
%\end{figure*}
%\subsubsection{Function Aggregation}
%Many time, the goal of a database query is to %summarize a table column based on some %\emph{aggregation function}. For example, one may %wish to compute the average hotel price in our %example table.
%
%To that end, we consider running the desired 

%\section{Fit in switch constraints}
%\minlan{How do you select which condition to check?}
%\ran{I don't have a good solution for that. I have this paragraph to explain how pruning can be %helpful even if exact filtering is infeasible. In practice, this is unlikely to happen as we can %support pretty complex expressions on multiple columns.}
%\ran{In theory, we can potentially run $\phi$ for a while (say, 10K entries) and then $\psi$ and see %which prunes better. This is only applicable to a scenario in which both are feasible within the %resource constraints and will require the switch CPU to change the datapath functionality. I think %that its better to avoid such solutions; perhaps the (outer) query planner can estimate which %expression would give better pruning and set the pipeline accordingly.}
%\ran{A different solution -- use $\phi$ for even entries and $\psi$ for odd ones. You'll get at least %50\% of the pruning of the best expression.}
%
\subsection{HAVING}
%\ran{unfortunately, our networking protocol almost kills this part, no more count min sketch for us :/. I'm wondering if we should even keep this}
%It is often useful to apply a filter based on the result of a stateful computation.
HAVING runs an aggregate function and filters \inputRows{} based on the results of the function. For example, 
%SELECT buyedID FROM Customers GROUP BY buyedID HAVING SUM(price) $>=$ 1000 can be used to compute all customers that have purchased at least $\$1000$ worth of products.
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT seller FROM Products GROUP BY seller HAVING MIN(price) < 6
\end{lstlisting}
should return (McCheetah, JellyFish).
%\begin{tabular}{c}
%                \hline
%                \seller\\\hline
%                    McCheetah\\
%                    JellyFish\\
%                \hline
%                \end{tabular}.\\
To address such queries (MIN(x) $<$ c or MAX(x) $>$ c), we check the condition on each incoming entry. If it is satisfied, we proceed to our Count Distinct solution (see \cref{sec:distinct}) -- if it reports that the current key 
%\minlan{do you mean key? try to use consistent terms with all the subsections before} \ran{Yes, sorry}
has not appeared before, we add it to the data structure and forward the packet; otherwise we prune it.

Other aggregation functions, such as COUNT or SUM are more challenging as a single entry is not enough for concluding whether we should pass the identifier. For example, one may ask which seller have items with a high total price:
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT seller FROM Products GROUP BY seller HAVING SUM(price) > 5
\end{lstlisting}
which may output
(McCheetah, Papizza).
%\begin{tabular}{c}
%                \hline
%                \seller\\\hline
%                    McCheetah\\
%                    Papizza\\
%                \hline
%                \end{tabular}.\\
%Alas, due to space and number-of-comparison constraints, the switch may not be able to aggregate every distinct entry value (e.g., seller in this example) separately due to its limited space. 

% We first stream the metadata\minlan{you used identifier, keys in other places} which contains the \inputCols{} on which the aggregation and computation is made. The switch stores all the metadata in a Count Min Sketch. uses the metadata to create a superset of all fields that should be output. 

\begin{figure*}[t]
    %\begin{tabular}{cc}
    \subfloat[Completion Time of Different Queries]{\label{fig:queries}\includegraphics[width =0.3\linewidth]
    {Figures/placeholder.png}}
    \subfloat[Distinct query delay breakdown]{\label{fig:breakdown}\includegraphics[width =0.3\linewidth]
    {Figures/placeholder.png}}
    %&
    %\hspace{-1mm}
\subfloat[Varying Number of Partitions (filtering query)]{\label{fig:vsNrWorkers}\includegraphics[width =0.32\linewidth]
    {Figures/End_to_End_Latency_PerNrWorkers.pdf}} 
    %\end{tabular}
    %\centering{
    %\includegraphics[width=\columnwidth]{Figures/legend}}
    \caption{\label{fig:prototype}\small The performance of \NAME{} vs. Spark SQL on filtering, \distinct, and \topn queries.}
%\vspace{-4mm}
\end{figure*}

Consider queries of the~form 
%SELECT x GROUP BY y Having $\Gamma(z)\ge c$ 
\begin{lstlisting}[backgroundcolor = \color{lightgray!50},style=SQL, breaklines=true]
SELECT x GROUP BY y Having f(z)>= c 
\end{lstlisting}
for \inputCol{} sets $x$ and $y$, an aggregation function $f\in\set{\COUNT,\SUM}$, an \inputCols{} $z$ (or nothing for COUNT), and $c\in\mathbb R$. The metadata stream contains $y$ and $z$ for each \inputRow{}.
We implement the Count-Min sketch which maintains counters for the metadata stream based on the function $f$. 
%whenever an \inputRow{} arrives we update it (by $1$ for \COUNT or by the value of $z$ for \SUM).
We then make a second pass (i.e., stream the data again)
%\minlan{what does second pass mean? You stream the data again?}\ran{Yes. The problem is that after sketching the data we get a subset of keys we need not to prune, but the data is not indexed by keys so we cannot simply request all rows that belong to these keys}
in which we prune all the keys for which the estimated $f(z)$ exceeds $c$. On the first pass, the switch blocks all packets and traffic only reaches the master node on the second pass.
Since the Count Min has one-sided error (i.e., it gives an estimator $\widetilde{f(z)}$ that satisfies $\widetilde{f(z)}\ge f(z)$),
%\minlan{what's one-side error? for people who don't know CM}, \ran{is this clear?}
we guarantee that every identifier $y$ for which $f(z)\ge c$ makes it to the worker. Thus, the estimation error only affects the pruning rate. We note that queries that ask for $f(z) < c$ (or have $f$ other than MIN/MAX/SUM/COUNT) are not currently supported by \NAME{}.
%\minlan{mention what function you do not support}\ran{Every function that is MIN/MAX/SUM/COUNT}


==> sections/theory.tex <==
\section{Theoretical Guarantees}\label{sec:analysis}

